Limit theorems for Random Walk excursion conditioned to have a typical area

We derive a functional central limit theorem for the excursion of a random walk conditioned on sweeping a prescribed geometric area. We assume that the increments of the random walk are integer-valued, centered, with a third moment equal to zero and a finite fourth moment. This result complements the work of \citep{DKW13} where local central limit theorems are provided for the geometric area of the excursion of a symmetric random walk with finite second moments. Our result turns out to be a key tool to derive the scaling limit of the \emph{Interacting Partially-Directed Self-Avoiding Walk} at criticality which is the object of a companion paper \citep{CarPet17a}. This requires to derive a reinforced version of our result in the case of a random walk with Laplace symmetric increments.

==> cnp.tex <==
@article {BDL09,
  AUTHOR =	 {Brak, R. and Dyke, P. and Lee, J. and Owczarek,
                  A. L. and Prellberg, T. and Rechnitzer, A. and
                  Whittington, S. G.},
  TITLE =	 {A self-interacting partially directed walk subject
                  to a force},
  JOURNAL =	 {J. Phys. A},
  FJOURNAL =	 {Journal of Physics. A. Mathematical and Theoretical},
  VOLUME =	 42,
  YEAR =	 2009,
  NUMBER =	 8,
  PAGES =	 {085001, 30},
  ISSN =	 {1751-8113},
  MRCLASS =	 {82B41 (82B44 82D60)},
  MRNUMBER =	 {2525477 (2010g:82028)},
  MRREVIEWER =	 {E. J. Janse van Rensburg},
  DOI =		 {10.1088/1751-8113/42/8/085001},
  URL =		 {http://dx.doi.org/10.1088/1751-8113/42/8/085001},
}

@book {MR2484222,
    AUTHOR = {Serfozo, Richard},
     TITLE = {Basics of applied stochastic processes},
    SERIES = {Probability and its Applications (New York)},
 PUBLISHER = {Springer-Verlag, Berlin},
      YEAR = {2009},
     PAGES = {xiv+443},
      ISBN = {978-3-540-89331-8},
   MRCLASS = {60-02 (60F05 60F15 60G07 60J10 60J65)},
  MRNUMBER = {2484222 (2010b:60003)},
MRREVIEWER = {Randall James Swift},
       DOI = {10.1007/978-3-540-89332-5},
       URL = {http://dx.doi.org/10.1007/978-3-540-89332-5},
}


@article {B76,
    AUTHOR = {Bolthausen, Erwin},
     TITLE = {On a functional central limit theorem for random walks
              conditioned to stay positive},
   JOURNAL = {Ann. Probability},
    VOLUME = {4},
      YEAR = {1976},
    NUMBER = {3},
     PAGES = {480--485},
   MRCLASS = {60B10},
  MRNUMBER = {0415702},
MRREVIEWER = {Douglas P. Kennedy},
}
	

@article {BOW90,
  AUTHOR =	 {Owczarek, A. L. and Binder, P. M. and Veal A.R and
                  Yeomans J.M.},
  TITLE =	 { Collapse transition in a simple polymer model:
                  exact results},
  JOURNAL =	 {J. Phys. A},
  FJOURNAL =	 {Journal of Physics. A. Mathematical and General},
  VOLUME =	 23,
  YEAR =	 1990,
  PAGES =	 {975--979},
}
@article{OP07,
  author =	 {Owczarek, A. L. and Prellberg, T.},
  title =	 {Exact solution of semi-flexible and super-flexible interacting partially directed walks},
  Journal =	 {J. Stat. Mech.: Theor. Exp.},
volume= {P11010},
  year =	 2007,
  pages =	 {1--14}
}

@article{OPB93,
  author =	 {Brak, R. and Owczarek, A. L. and Prellberg, T.},
  title =	 {The tricritical behavior of self-interacting
                  partially directed walks.},
  Journal =	 {Journal of Statistical Physics},
  Volume =	 72,
  year =	 1993,
  pages =	 {737--772}
}

@article{POBG93,
  author =	 {Brak, R. and Owczarek, A. L. and Prellberg, T. and
                  Guttmann, A. J.},
  title =	 {Finite-length scaling of collapsing directed walks},
  Journal =	 {Phys. Rev. E},
  Volume =	 48,
  number =	 4,
  year =	 1993,
  pages =	 {2386--2396}
}


@incollection {CHP12,
  AUTHOR =	 {Caravenna, Francesco and den Hollander, Frank and
                  P{\'e}tr{\'e}lis, Nicolas},
  TITLE =	 {Lectures on random polymers},
  BOOKTITLE =	 {Probability and statistical physics in two and more
                  dimensions},
  SERIES =	 {Clay Math. Proc.},
  VOLUME =	 15,
  PAGES =	 {319--393},
  PUBLISHER =	 {Amer. Math. Soc.},
  ADDRESS =	 {Providence, RI},
  YEAR =	 2012,
  MRCLASS =	 {60K37 (60F10 82B26 82D60 92D20)},
  MRNUMBER =	 3025394,
  MRREVIEWER =	 {Stavros Vakeroudis},
}


@Book {Bill08,
title = {Convergence of Probability Measures},
author = {Billingsley, Patrick},
publisher = {John Wiley and Sons, Inc.},
 address = {New York},
isbn = {9780470316962},
url = {http://dx.doi.org/10.1002/9780470316962.fmatter},
doi = {10.1002/9780470316962.fmatter},
pages = {I--IX},
mrnumber = {MR1700749 (2000e:60008)},
booktitle = {Convergence of Probability Measures},
year = {2008},
}








@book {DZ,
  AUTHOR =	 {Dembo, Amir and Zeitouni, Ofer},
  TITLE =	 {Large deviations techniques and applications},
  SERIES =	 {Stochastic Modelling and Applied Probability},
  VOLUME =	 38,
  NOTE =	 {Corrected reprint of the second (1998) edition},
  PUBLISHER =	 {Springer-Verlag},
  ADDRESS =	 {Berlin},
  YEAR =	 2010,
  PAGES =	 {xvi+396},
  ISBN =	 {978-3-642-03310-0},
  MRCLASS =	 {60F10},
  MRNUMBER =	 {2571413 (2011b:60094)},
  DOI =		 {10.1007/978-3-642-03311-7},
  URL =		 {http://dx.doi.org/10.1007/978-3-642-03311-7},
}





@article {MR2197112,
    AUTHOR = {Caravenna, Francesco},
     TITLE = {A local limit theorem for random walks conditioned to stay
              positive},
   JOURNAL = {Probab. Theory Related Fields},
  FJOURNAL = {Probability Theory and Related Fields},
    VOLUME = {133},
      YEAR = {2005},
    NUMBER = {4},
     PAGES = {508--530},
      ISSN = {0178-8051},
     CODEN = {PTRFEU},
   MRCLASS = {60G50 (60F05 60K05)},
  MRNUMBER = {2197112 (2006k:60077)},
MRREVIEWER = {No{\"e}l Veraverbeke},
       DOI = {10.1007/s00440-005-0444-5},
       URL = {http://dx.doi.org/10.1007/s00440-005-0444-5},
}
@article {CapMarTon12,
    AUTHOR = {Caputo, Pietro and Martinelli, Fabio and Toninelli, Fabio
              Lucio},
     TITLE = {Mixing times of monotone surfaces and {SOS} interfaces: a mean
              curvature approach},
   JOURNAL = {Comm. Math. Phys.},
  FJOURNAL = {Communications in Mathematical Physics},
    VOLUME = {311},
      YEAR = {2012},
    NUMBER = {1},
     PAGES = {157--189},
      ISSN = {0010-3616},
     CODEN = {CMPHAY},
   MRCLASS = {82C24 (60J27)},
  MRNUMBER = {2892467},
MRREVIEWER = {Nicoletta Cancrini},
       DOI = {10.1007/s00220-012-1425-z},
       URL = {http://dx.doi.org/10.1007/s00220-012-1425-z},
}

@book {DZ,
  AUTHOR =	 {Dembo, Amir and Zeitouni, Ofer},
  TITLE =	 {Large deviations techniques and applications},
  SERIES =	 {Stochastic Modelling and Applied Probability},
  VOLUME =	 38,
  NOTE =	 {Corrected reprint of the second (1998) edition},
  PUBLISHER =	 {Springer-Verlag},
  ADDRESS =	 {Berlin},
  YEAR =	 2010,
  PAGES =	 {xvi+396},
  ISBN =	 {978-3-642-03310-0},
  MRCLASS =	 {60F10},
  MRNUMBER =	 {2571413 (2011b:60094)},
  DOI =		 {10.1007/978-3-642-03311-7},
  URL =		 {http://dx.doi.org/10.1007/978-3-642-03311-7},
}

@article {DH96,
  AUTHOR =	 {Dobrushin, R. and Hryniv, O.},
  TITLE =	 {Fluctuations of shapes of large areas under paths of
                  random walks},
  JOURNAL =	 {Probab. Theory Related Fields},
  FJOURNAL =	 {Probability Theory and Related Fields},
  VOLUME =	 105,
  YEAR =	 1996,
  NUMBER =	 4,
  PAGES =	 {423--458},
  ISSN =	 {0178-8051},
  CODEN =	 {PTRFEU},
  MRCLASS =	 {60F17 (60F10 60J15 82B24)},
  MRNUMBER =	 {1402652 (97h:60029)},
  MRREVIEWER =	 {Christian Maes},
  DOI =		 {10.1007/BF01191908},
  URL =		 {http://dx.doi.org/10.1007/BF01191908},
}

@book {RD05,
  AUTHOR =	 {Durrett, Rick},
  TITLE =	 {Probability: theory and examples},
  SERIES =	 {Cambridge Series in Statistical and Probabilistic
                  Mathematics},
  EDITION =	 {Fourth},
  PUBLISHER =	 {Cambridge University Press},
  ADDRESS =	 {Cambridge},
  YEAR =	 2010,
  PAGES =	 {x+428},
  ISBN =	 {978-0-521-76539-8},
  MRCLASS =	 {60-01},
  MRNUMBER =	 {2722836 (2011e:60001)},
}

@book {cf:Gia,
  AUTHOR =	 {Giacomin, Giambattista},
  TITLE =	 {Random polymer models},
  PUBLISHER =	 {Imperial College Press},
  ADDRESS =	 {London},
  YEAR =	 2007,
  PAGES =	 {xvi+242},
  ISBN =	 {978-1-86094-786-5; 1-86094-786-7},
  MRCLASS =	 {82B44 (82-02 82B41 82D60)},
  MRNUMBER =	 {2380992 (2009c:82025)},
  MRREVIEWER =	 {Stuart G. Whittington},
  DOI =		 {10.1142/9781860948299},
  URL =		 {http://dx.doi.org/10.1142/9781860948299},
}

@book {GIA11,
    AUTHOR = {Giacomin, Giambattista},
     TITLE = {Disorder and critical phenomena through basic probability
              models},
    SERIES = {Lecture Notes in Mathematics},
    VOLUME = {2025},
      NOTE = {Lecture notes from the 40th Probability Summer School held in
              Saint-Flour, 2010,
              {\'E}cole d'{\'E}t{\'e} de Probabilit{\'e}s de Saint-Flour.
              [Saint-Flour Probability Summer School]},
 PUBLISHER = {Springer},
   ADDRESS = {Heidelberg},
      YEAR = {2011},
     PAGES = {xii+130},
      ISBN = {978-3-642-21155-3},
   MRCLASS = {82B44 (60K05 60K35 82-02 82B27)},
  MRNUMBER = {2816225 (2012g:82027)},
MRREVIEWER = {Rongfeng Sun},
       DOI = {10.1007/978-3-642-21156-0},
       URL = {http://dx.doi.org/10.1007/978-3-642-21156-0},
}


@article {J07,
  AUTHOR =	 {Janson, Svante},
  TITLE =	 {Brownian excursion area, {W}right's constants in
                  graph enumeration, and other {B}rownian areas},
  JOURNAL =	 {Probab. Surv.},
  FJOURNAL =	 {Probability Surveys},
  VOLUME =	 4,
  YEAR =	 2007,
  PAGES =	 {80--145},
  ISSN =	 {1549-5787},
  MRCLASS =	 {60J65},
  MRNUMBER =	 {2318402 (2008d:60106)},
}

@article {K46,
  AUTHOR =	 {Kac, M.},
  TITLE =	 {On the average of a certain {W}iener functional and
                  a related limit theorem in calculus of probability},
  JOURNAL =	 {Trans. Amer. Math. Soc.},
  FJOURNAL =	 {Transactions of the American Mathematical Society},
  VOLUME =	 59,
  YEAR =	 1946,
  PAGES =	 {401--414},
  ISSN =	 {0002-9947},
  MRCLASS =	 {60.0X},
  MRNUMBER =	 {0016570 (8,37b)},
  MRREVIEWER =	 {M. Lo{\`e}ve},
}

@article {NGP13,
  AUTHOR =	 {Nguyen, Gia Bao and P{\'e}tr{\'e}lis, Nicolas},
  TITLE =	 {A variational formula for the free energy of the
                  partially directed polymer collapse},
  JOURNAL =	 {J. Stat. Phys.},
  FJOURNAL =	 {Journal of Statistical Physics},
  VOLUME =	 151,
  YEAR =	 2013,
  NUMBER =	 6,
  PAGES =	 {1099--1120},
  ISSN =	 {0022-4715},
  MRCLASS =	 {82D60 (82B26 82B41)},
  MRNUMBER =	 3063498,
  MRREVIEWER =	 {Stuart G. Whittington},
  DOI =		 {10.1007/s10955-013-0748-2},
  URL =		 {http://dx.doi.org/10.1007/s10955-013-0748-2},
}

@incollection {Sa80,
  AUTHOR =	 {Sakhanenko, A. I.},
  TITLE =	 {On unimprovable estimates of the rate of convergence
                  in the invariance principle},
  BOOKTITLE =	 {Colloq. Math. Soc. J\'anos Bolyai},
  SERIES =	 { Nonparametric Statistical Inference},
  VOLUME =	 32,
  PAGES =	 { 779--783},
  ADDRESS =	 {Budapest, Hungary},
  YEAR =	 1980,
}

@article {Sh95,
  AUTHOR =	 {Shao, Qi Man},
  TITLE =	 {Strong approximation theorems for independent random
                  variables and their applications},
  JOURNAL =	 {J. Multivariate Anal.},
  FJOURNAL =	 {Journal of Multivariate Analysis},
  VOLUME =	 52,
  YEAR =	 1995,
  NUMBER =	 1,
  PAGES =	 {107--130},
  ISSN =	 {0047-259X},
  MRCLASS =	 {60F17 (60F15 60G50)},
  MRNUMBER =	 {1325373 (96c:60047)},
  MRREVIEWER =	 {Thomas Mikosch},
  DOI =		 {10.1006/jmva.1995.1006},
  URL =		 {http://dx.doi.org/10.1006/jmva.1995.1006},
}

@article{HST13,
  author =	 {Samanta, H.S. and Thirumalai, D.},
  title =	 {Exact solution of the {Zwanzig-Lauritzen} model of
                  polymer crystallization under tension},
  journal =	 {J. Chem. Phys.},
  volume =	 138,
  pages =	 104901,
  year =	 2013
}

@article{ZL68,
  author =	 {Zwanzig, R. and Lauritzen, J.I.},
  title =	 {Exact calculation of the partition function for a
                  model of two dimensional polymer crystallization by
                  chain folding},
  journal =	 {J. Chem. Phys.},
  volume =	 48,
number = 8,
  pages =	 3351,
  year =	 1968,
}

@article{S13,
author = "Sohier, Julien",
doi = "10.1214/11-AIHP456",
fjournal = "Annales de l'Institut Henri Poincaré, Probabilités et Statistiques",
journal = "Ann. Inst. H. Poincar\'e  Probab. Statist.",
month = "05",
number = "2",
pages = "483--505",
publisher = "Institut Henri Poincaré",
title = "The scaling limits of a heavy tailed Markov renewal process",
url = "http://dx.doi.org/10.1214/11-AIHP456",
volume = "49",
year = "2013"
}



@article {HV04,
    AUTHOR = {Hryniv, O. and Velenik, Y.},
     TITLE = {Universality of critical behaviour in a class of recurrent
              random walks},
   JOURNAL = {Probab. Theory Related Fields},
  FJOURNAL = {Probability Theory and Related Fields},
    VOLUME = {130},
      YEAR = {2004},
    NUMBER = {2},
     PAGES = {222--258},
      ISSN = {0178-8051},
     CODEN = {PTRFEU},
   MRCLASS = {82B24 (60J10 82B27 82B41)},
  MRNUMBER = {2093763 (2005i:82028)},
MRREVIEWER = {Bernard Ycart},
       DOI = {10.1007/s00440-004-0353-z},
       URL = {http://dx.doi.org/10.1007/s00440-004-0353-z},
}
	
@article {AbSm86,
    AUTHOR = {Abraham, D. B. and Smith, E. R.},
     TITLE = {An exactly solved model with a wetting transition},
   JOURNAL = {J. Statist. Phys.},
  FJOURNAL = {Journal of Statistical Physics},
    VOLUME = {43},
      YEAR = {1986},
    NUMBER = {3-4},
     PAGES = {621--643},
      ISSN = {0022-4715},
     CODEN = {JSTPSB},
   MRCLASS = {82A25},
  MRNUMBER = {845731 (87i:82036)},
MRREVIEWER = {M. Lawrence Glasser},
       DOI = {10.1007/BF01020656},
       URL = {http://dx.doi.org/10.1007/BF01020656},
}
	

@Unpublished{NT14,
  author = 	 {Torri, Niccolo},
  title = 	 {Pinning model with heavy tailed disorder},
  note = 	 {Private communication},
  OPTkey = 	 {},
  OPTmonth = 	 {February},
  year = 	 {2014},
  OPTannote = 	 {}
}

@article {TA93,
    AUTHOR = {Tak{\'a}cs, Lajos},
     TITLE = {On the distribution of the integral of the absolute value of
              the {B}rownian motion},
   JOURNAL = {Ann. Appl. Probab.},
  FJOURNAL = {The Annals of Applied Probability},
    VOLUME = {3},
      YEAR = {1993},
    NUMBER = {1},
     PAGES = {186--197},
      ISSN = {1050-5164},
   MRCLASS = {60J65 (60G15)},
  MRNUMBER = {1202522 (93i:60154)}
}
	



@article {IS98,
    AUTHOR = {Ioffe, Dmitry and Schonmann, Roberto H.},
     TITLE = {Dobrushin-{K}oteck\'y-{S}hlosman theorem up to the critical
              temperature},
   JOURNAL = {Comm. Math. Phys.},
  FJOURNAL = {Communications in Mathematical Physics},
    VOLUME = {199},
      YEAR = {1998},
    NUMBER = {1},
     PAGES = {117--167},
      ISSN = {0010-3616},
     CODEN = {CMPHAY},
   MRCLASS = {82B05 (60F10 60K35 82B20 82B26)},
  MRNUMBER = {1660207 (2000f:82003)},
MRREVIEWER = {Francis Comets},
       DOI = {10.1007/s002200050497},
       URL = {http://dx.doi.org/10.1007/s002200050497},
}
		

@article {I95,
    AUTHOR = {Ioffe, Dmitry},
     TITLE = {Exact large deviation bounds up to {$T_c$} for the {I}sing
              model in two dimensions},
   JOURNAL = {Probab. Theory Related Fields},
  FJOURNAL = {Probability Theory and Related Fields},
    VOLUME = {102},
      YEAR = {1995},
    NUMBER = {3},
     PAGES = {313--330},
      ISSN = {0178-8051},
     CODEN = {PTRFEU},
   MRCLASS = {60F10 (60K35 82B20 82B24 82B43)},
  MRNUMBER = {1339736 (97f:60063)},
       DOI = {10.1007/BF01192464},
       URL = {http://dx.doi.org/10.1007/BF01192464},
}
		

@article {I94,
    AUTHOR = {Ioffe, Dmitry},
     TITLE = {Large deviations for the {$2$}{D} {I}sing model: a lower bound
              without cluster expansions},
   JOURNAL = {J. Statist. Phys.},
  FJOURNAL = {Journal of Statistical Physics},
    VOLUME = {74},
      YEAR = {1994},
    NUMBER = {1-2},
     PAGES = {411--432},
      ISSN = {0022-4715},
     CODEN = {JSTPSB},
   MRCLASS = {82B20 (60F10)},
  MRNUMBER = {1257822 (95a:82017)},
MRREVIEWER = {Flora Koukiou},
       DOI = {10.1007/BF02186818},
       URL = {http://dx.doi.org/10.1007/BF02186818},
}
		
@book {DKS92,
    AUTHOR = {Dobrushin, R. and Koteck{\'y}, R. and Shlosman, S.},
     TITLE = {Wulff construction},
    SERIES = {Translations of Mathematical Monographs},
    VOLUME = {104},
      NOTE = {A global shape from local interaction,
              Translated from the Russian by the authors},
 PUBLISHER = {American Mathematical Society},
   ADDRESS = {Providence, RI},
      YEAR = {1992},
     PAGES = {x+204},
      ISBN = {0-8218-4563-2},
   MRCLASS = {82B05 (82-02 82B20)},
  MRNUMBER = {1181197 (93k:82002)},
MRREVIEWER = {Jo{\"e}l De Coninck},
}
	
@article{W1901,
author={Wulff, G.},
title={Zur frage der Geschwindigkeit des Wachstums und der auflosüng der krystallflagen},
journal={Z. Kryst. Mineral.},
volume=34,
year=1901,
pages={449}
}
 @article {HDHK03,
    AUTHOR = {van der Hofstad, Remco and den Hollander, Frank and K{\"o}nig,
              Wolfgang},
     TITLE = {Weak interaction limits for one-dimensional random polymers},
   JOURNAL = {Probab. Theory Related Fields},
  FJOURNAL = {Probability Theory and Related Fields},
    VOLUME = {125},
      YEAR = {2003},
    NUMBER = {4},
     PAGES = {483--521},
      ISSN = {0178-8051},
     CODEN = {PTRFEU},
   MRCLASS = {60F05 (60F10 82D60)},
  MRNUMBER = {1974412 (2004e:60038)},
MRREVIEWER = {David J. Aldous},
       DOI = {10.1007/s00440-002-0248-9},
       URL = {http://dx.doi.org/10.1007/s00440-002-0248-9},
}
	

@book {Asmussen03,
    AUTHOR = {Asmussen, S{\o}ren},
     TITLE = {Applied probability and queues},
    SERIES = {Applications of Mathematics (New York)},
    VOLUME = {51},
   EDITION = {Second},
      NOTE = {Stochastic Modelling and Applied Probability},
 PUBLISHER = {Springer-Verlag},
   ADDRESS = {New York},
      YEAR = {2003},
     PAGES = {xii+438},
      ISBN = {0-387-00211-1},
   MRCLASS = {60-02 (60K25 60K30 90B15 90B22)},
  MRNUMBER = {1978607 (2004f:60001)},
MRREVIEWER = {Jozef L. Teugels},
}
@article {AS06,
    AUTHOR = {Alexander, Kenneth S. and Sidoravicius, Vladas},
     TITLE = {Pinning of polymers and interfaces by random potentials},
   JOURNAL = {Ann. Appl. Probab.},
  FJOURNAL = {The Annals of Applied Probability},
    VOLUME = {16},
      YEAR = {2006},
    NUMBER = {2},
     PAGES = {636--669},
      ISSN = {1050-5164},
   MRCLASS = {60K35 (82B44 82D60)},
  MRNUMBER = {2244428 (2007i:60126)},
MRREVIEWER = {Giambattista Giacomin},
       DOI = {10.1214/105051606000000015},
       URL = {http://dx.doi.org/10.1214/105051606000000015},
}
		
@article {DGLT09,
    AUTHOR = {Derrida, Bernard and Giacomin, Giambattista and Lacoin, Hubert
              and Toninelli, Fabio Lucio},
     TITLE = {Fractional moment bounds and disorder relevance for pinning
              models},
   JOURNAL = {Comm. Math. Phys.},
  FJOURNAL = {Communications in Mathematical Physics},
    VOLUME = {287},
      YEAR = {2009},
    NUMBER = {3},
     PAGES = {867--887},
      ISSN = {0010-3616},
     CODEN = {CMPHAY},
   MRCLASS = {82B44 (60K05 60K37)},
  MRNUMBER = {2486665 (2010a:82029)},
MRREVIEWER = {Rongfeng Sun},
       DOI = {10.1007/s00220-009-0737-0},
       URL = {http://dx.doi.org/10.1007/s00220-009-0737-0},
}


@article{DHV92,
year=1992,
issn={0022-4715},
journal={Journal of Statistical Physics},
volume=66,
number={5-6},
doi={10.1007/BF01054419},
title={Effect of disorder on two-dimensional wetting},
url={http://dx.doi.org/10.1007/BF01054419},
publisher={Kluwer Academic Publishers-Plenum Publishers},
keywords={Wetting transition; disorder; transfer matrix},
author={Derrida, B. and Hakim, V. and Vannimenus, J.},
pages={1189-1213},
language={English}
}
@book {Bi,
    AUTHOR = {Billingsley, Patrick},
     TITLE = {Convergence of probability measures},
    SERIES = {Wiley Series in Probability and Statistics: Probability and
              Statistics},
   EDITION = {Second},
      NOTE = {A Wiley-Interscience Publication},
 PUBLISHER = {John Wiley \& Sons, Inc., New York},
      YEAR = {1999},
     PAGES = {x+277},
      ISBN = {0-471-19745-9},
   MRCLASS = {60B10 (28A33 60F17)},
  MRNUMBER = {1700749 (2000e:60008)},
       DOI = {10.1002/9780470316962},
       URL = {http://dx.doi.org/10.1002/9780470316962},
}
	


@book {W,
    AUTHOR = {Williams, David},
     TITLE = {Probability with martingales},
    SERIES = {Cambridge Mathematical Textbooks},
 PUBLISHER = {Cambridge University Press, Cambridge},
      YEAR = {1991},
     PAGES = {xvi+251},
      ISBN = {0-521-40455-X; 0-521-40605-6},
   MRCLASS = {60-01 (60G42)},
  MRNUMBER = {1155402 (93d:60002)},
MRREVIEWER = {Jia Gang Wang},
}

@article{CNGP13,
author = "Carmona, Philippe and Nguyen, Gia Bao and P\'etr\'elis, Nicolas",
doi = "10.1214/15-AOP1046",
fjournal = "The Annals of Probability",
journal = "Ann. Probab.",
month = "09",
number = "5",
pages = "3234--3290",
publisher = "The Institute of Mathematical Statistics",
title = "Interacting partially directed self avoiding walk. From phase transition to the geometry of the collapsed phase",
url = "http://dx.doi.org/10.1214/15-AOP1046",
volume = "44",
year = "2016"
}





@article{POBG93,
  author =	 {Brak, R. and Owczarek, A. L. and Prellberg, T. and
                  Guttmann, A. J.},
  title =	 {Finite-length scaling of collapsing directed walks},
  Journal =	 {Phys. Rev. E},
  Volume =	 48,
  number =	 4,
  year =	 1993,
  pages =	 {2386--2396}
}

@article {BGW92,
  AUTHOR =	 {Brak, R. and Guttmann, A. J. and Whittington, S. G.},
  TITLE =	 {A collapse transition in a directed walk model},
  JOURNAL =	 {J. Phys. A},
  FJOURNAL =	 {Journal of Physics. A. Mathematical and General},
  VOLUME =	 25,
  YEAR =	 1992,
  NUMBER =	 9,
  PAGES =	 {2437--2446},
  ISSN =	 {0305-4470},
  CODEN =	 {JPHAC5},
  MRCLASS =	 {82B41 (82D60)},
  MRNUMBER =	 {1164357 (93a:82025)},
  URL =		 {http://stacks.iop.org/0305-4470/25/2437},
}






@book {MR1083357,
    AUTHOR = {Revuz, Daniel and Yor, Marc},
     TITLE = {Continuous martingales and {B}rownian motion},
    SERIES = {Grundlehren der Mathematischen Wissenschaften [Fundamental
              Principles of Mathematical Sciences]},
    VOLUME = {293},
 PUBLISHER = {Springer-Verlag, Berlin},
      YEAR = {1991},
     PAGES = {x+533},
      ISBN = {3-540-52167-4},
   MRCLASS = {60G48 (60G44 60H05 60H10)},
  MRNUMBER = {1083357 (92d:60053)},
MRREVIEWER = {F. B. Knight},
}
@book {RY91,
    AUTHOR = {Revuz, Daniel and Yor, Marc},
     TITLE = {Continuous martingales and {B}rownian motion},
    SERIES = {Grundlehren der Mathematischen Wissenschaften [Fundamental
              Principles of Mathematical Sciences]},
    VOLUME = {293},
 PUBLISHER = {Springer-Verlag, Berlin},
      YEAR = {1991},
     PAGES = {x+533},
      ISBN = {3-540-52167-4},
   MRCLASS = {60G48 (60G44 60H05 60H10)},
  MRNUMBER = {1083357 (92d:60053)},
MRREVIEWER = {F. B. Knight},
}
@article {DONEY97,
    AUTHOR = {Doney, R. A.},
     TITLE = {One-sided local large deviation and renewal theorems in the
              case of infinite mean},
   JOURNAL = {Probab. Theory Related Fields},
  FJOURNAL = {Probability Theory and Related Fields},
    VOLUME = {107},
      YEAR = {1997},
    NUMBER = {4},
     PAGES = {451--465},
      ISSN = {0178-8051},
     CODEN = {PTRFEU},
   MRCLASS = {60F10 (60J15 60K05)},
  MRNUMBER = {1440141 (98e:60040)},
MRREVIEWER = {No{\"e}l Veraverbeke},
       DOI = {10.1007/s004400050093},
       URL = {http://dx.doi.org/10.1007/s004400050093},
}

@article {Kes63,
    AUTHOR = {Kesten, Harry},
     TITLE = {Ratio theorems for random walks. {II}},
   JOURNAL = {J. Analyse Math.},
  FJOURNAL = {Journal d'Analyse Math\'ematique},
    VOLUME = {11},
      YEAR = {1963},
     PAGES = {323--379},
      ISSN = {0021-7670},
   MRCLASS = {60.66},
  MRNUMBER = {0163365 (29 \#668)},
MRREVIEWER = {J. Gillis},
}
@article {DKW13,
    AUTHOR = {Denisov, Denis and Kolb, Martin and Wachtel, Vitali},
     TITLE = {Local asymptotics for the area of random walk excursions},
   JOURNAL = {J. Lond. Math. Soc. (2)},
  FJOURNAL = {Journal of the London Mathematical Society. Second Series},
    VOLUME = {91},
      YEAR = {2015},
    NUMBER = {2},
     PAGES = {495--513},
      ISSN = {0024-6107},
   MRCLASS = {60G50 (60F17 60G40)},
  MRNUMBER = {3355112},
       DOI = {10.1112/jlms/jdu078},
       URL = {http://dx.doi.org/10.1112/jlms/jdu078},
}	


@book {IL71,
    AUTHOR = {Ibragimov, I. A. and Linnik, Yu. V.},
     TITLE = {Independent and stationary sequences of random variables},
      NOTE = {With a supplementary chapter by I. A. Ibragimov and V. V.
              Petrov,
              Translation from the Russian edited by J. F. C. Kingman},
 PUBLISHER = {Wolters-Noordhoff Publishing, Groningen},
      YEAR = {1971},
     PAGES = {443},
   MRCLASS = {60FXX},
  MRNUMBER = {0322926 (48 \#1287)},
}

@article {CD08,
    AUTHOR = {Caravenna, Francesco and Deuschel, Jean-Dominique},
     TITLE = {Pinning and wetting transition for {$(1+1)$}-dimensional
              fields with {L}aplacian interaction},
   JOURNAL = {Ann. Probab.},
  FJOURNAL = {The Annals of Probability},
    VOLUME = {36},
      YEAR = {2008},
    NUMBER = {6},
     PAGES = {2388--2433},
      ISSN = {0091-1798},
     CODEN = {APBYAE},
   MRCLASS = {60K35 (60F05 82B41)},
  MRNUMBER = {2478687 (2010e:60206)},
       DOI = {10.1214/08-AOP395},
       URL = {http://dx.doi.org/10.1214/08-AOP395},
}

@article {CD09,
    AUTHOR = {Caravenna, Francesco and Deuschel, Jean-Dominique},
     TITLE = {Scaling limits of {$(1+1)$}-dimensional pinning models with
              {L}aplacian interaction},
   JOURNAL = {Ann. Probab.},
  FJOURNAL = {The Annals of Probability},
    VOLUME = {37},
      YEAR = {2009},
    NUMBER = {3},
     PAGES = {903--945},
      ISSN = {0091-1798},
     CODEN = {APBYAE},
   MRCLASS = {60K35 (60F05 82B41)},
  MRNUMBER = {2537545 (2010j:60237)},
MRREVIEWER = {Zhong Gen Su},
       DOI = {10.1214/08-AOP424},
       URL = {http://dx.doi.org/10.1214/08-AOP424},
}

@article {A01,
    AUTHOR = {Alexander, Kenneth S.},
     TITLE = {Cube-root boundary fluctuations for droplets in random cluster
              models},
   JOURNAL = {Comm. Math. Phys.},
  FJOURNAL = {Communications in Mathematical Physics},
    VOLUME = {224},
      YEAR = {2001},
    NUMBER = {3},
     PAGES = {733--781},
      ISSN = {0010-3616},
     CODEN = {CMPHAY},
   MRCLASS = {82B43 (60K35)},
  MRNUMBER = {1871907 (2003i:82041)},
       DOI = {10.1007/s220-001-8022-2},
       URL = {http://dx.doi.org/10.1007/s220-001-8022-2},
}

@book {Ber96,
    AUTHOR = {Bertoin, Jean},
     TITLE = {L\'evy processes},
    SERIES = {Cambridge Tracts in Mathematics},
    VOLUME = {121},
 PUBLISHER = {Cambridge University Press, Cambridge},
      YEAR = {1996},
     PAGES = {x+265},
      ISBN = {0-521-56243-0},
   MRCLASS = {60J30 (60J55)},
  MRNUMBER = {1406564 (98e:60117)},
MRREVIEWER = {Patrick Fitzsimmons},
}

@book {cf:dH,
    AUTHOR = {den Hollander, Frank},
     TITLE = {Random polymers},
    SERIES = {Lecture Notes in Mathematics},
    VOLUME = {1974},
      NOTE = {Lectures from the 37th Probability Summer School held in
              Saint-Flour, 2007},
 PUBLISHER = {Springer-Verlag, Berlin},
      YEAR = {2009},
     PAGES = {xiv+258},
      ISBN = {978-3-642-00332-5},
   MRCLASS = {60K35 (60-02 60F10 60F17 60G50 60K37 82B26 82B41)},
  MRNUMBER = {2504175 (2010h:60265)},
MRREVIEWER = {Rongfeng Sun},
       DOI = {10.1007/978-3-642-00333-2},
       URL = {http://dx.doi.org/10.1007/978-3-642-00333-2},
}



@Book{Flory,
  author = 	 {Flory, Paul J.},
  title = 	 {Principles of Polymer chemistry},
  publisher = 	 {Cornell University Press},
  year = 	 1953,
  address = 	 {Ithaca (NY)}}

@Unpublished{CSZ,
  author = 	 {Caravenna, F. and Sun, R. and Zygouras, N.},
  title = 	 {The continuum disordered pinning model},
  note = 	 {http://arxiv.org/abs/1406.5088 (math.PR), submitted},
  url = {http://arxiv.org/abs/1406.5088}

}

@Article{DGZ05,
  author = 	 {Deuschel, J.D. and Giacomin, G. and Zambotti, L.},
  title = 	 { Scaling limits of equilibrium wetting models in (1 + 1)-dimension},
  journal = 	 {Probab. Theory Related Fields},
  year = 	 2005,
  volume = 	 132,
  number = 	 4,
      ISSN = {0178-8051},
     CODEN = {PTRFEU},
   MRCLASS = {60K35 (60F10 82B41)},
  MRNUMBER = {2198199 (2007f:60080)},
MRREVIEWER = {Peter Eichelsbacher},
       DOI = {10.1007/s00440-004-0401-8},
       URL = {http://dx.doi.org/10.1007/s00440-004-0401-8}
}

@article {CGZ06,
    AUTHOR = {Caravenna, Francesco and Giacomin, Giambattista and Zambotti,
              Lorenzo},
     TITLE = {Sharp asymptotic behavior for wetting models in
              {$(1+1)$}-dimension},
   JOURNAL = {Electron. J. Probab.},
  FJOURNAL = {Electronic Journal of Probability},
    VOLUME = {11},
      YEAR = {2006},
     PAGES = {no. 14, 345--362 (electronic)},
      ISSN = {1083-6489},
   MRCLASS = {60K10 (60K05)},
  MRNUMBER = {2217821 (2007c:60091)},
MRREVIEWER = {No{\"e}l Veraverbeke},
       DOI = {10.1214/EJP.v11-320},
       URL = {http://dx.doi.org/10.1214/EJP.v11-320},
}

@Unpublished{GT,
  author = 	 {Guttmann, Anthony J},
  title = 	 {Analysis of series expansions for non-algebraic singularities},
  note = 	 {submitted, arXiv:1405.5327 [math.PH]},
  OPTkey = 	 {},
  OPTmonth = 	 {},
  OPTyear = 	 {2014},
  OPTannote = 	 {}
}

@article {DH97,
    AUTHOR = {Dobrushin, R. and Hryniv, O.},
     TITLE = {Fluctuations of the phase boundary in the {$2$}{D} {I}sing
              ferromagnet},
   JOURNAL = {Comm. Math. Phys.},
  FJOURNAL = {Communications in Mathematical Physics},
    VOLUME = {189},
      YEAR = {1997},
    NUMBER = {2},
     PAGES = {395--445},
      ISSN = {0010-3616},
     CODEN = {CMPHAY},
   MRCLASS = {82B24 (60F05 60K35 82B20 82B41)},
  MRNUMBER = {1480026 (99a:82037)},
MRREVIEWER = {Marek Biskup},
       DOI = {10.1007/s002200050209},
       URL = {http://dx.doi.org/10.1007/s002200050209},
}

@book {LL10,
    AUTHOR = {Lawler, Gregory F. and Limic, Vlada},
     TITLE = {Random walk: a modern introduction},
    SERIES = {Cambridge Studies in Advanced Mathematics},
    VOLUME = {123},
 PUBLISHER = {Cambridge University Press, Cambridge},
      YEAR = {2010},
     PAGES = {xii+364},
      ISBN = {978-0-521-51918-2},
   MRCLASS = {60G50 (60-02)},
  MRNUMBER = {2677157 (2012a:60132)},
MRREVIEWER = {Andrew R. Wade},
       DOI = {10.1017/CBO9780511750854},
       URL = {http://dx.doi.org/10.1017/CBO9780511750854},
}

@article{PT17,
  author = 	 {P\'etr\'elis, N. and Torri, N.},
  title = 	 {Collapse transition of the interacting prudent walk},
  note = 	 {https://arxiv.org/abs/1610.07542 (math.PR), submitted},
  url = {https://arxiv.org/abs/1610.07542}
}


@article {MR3343288,
    AUTHOR = {Sohier, Julien},
     TITLE = {The scaling limits of the non critical strip wetting model},
   JOURNAL = {Stochastic Process. Appl.},
  FJOURNAL = {Stochastic Processes and their Applications},
    VOLUME = {125},
      YEAR = {2015},
    NUMBER = {8},
     PAGES = {3075--3103},
      ISSN = {0304-4149},
   MRCLASS = {60K15 (60F17 60G50 60K05 60K20 60K35 82B27)},
  MRNUMBER = {3343288},
       DOI = {10.1016/j.spa.2015.02.012},
       URL = {http://dx.doi.org/10.1016/j.spa.2015.02.012},
}

@Unpublished{S14,
  author = 	 {Sohier, Julien},
  title = 	 {The scaling limits of the non critical strip wetting model},
  note = 	 {submitted, arXiv:1406.3604 [math.PR]},
  OPTkey = 	 {},
  OPTmonth = 	 {},
  OPTyear = 	 {2014},
  OPTannote = 	 {}
}

@article {CD12009,
    AUTHOR = {Caravenna, Francesco and Deuschel, Jean-Dominique},
     TITLE = {Pinning and wetting transition for {$(1+1)$}-dimensional
              fields with {L}aplacian interaction},
   JOURNAL = {Ann. Probab.},
  FJOURNAL = {The Annals of Probability},
    VOLUME = {36},
      YEAR = {2008},
    NUMBER = {6},
     PAGES = {2388--2433},
      ISSN = {0091-1798},
     CODEN = {APBYAE},
   MRCLASS = {60K35 (60F05 82B41)},
  MRNUMBER = {2478687 (2010e:60206)},
       DOI = {10.1214/08-AOP395},
       URL = {http://dx.doi.org/10.1214/08-AOP395},
}

@article {MR1340834,
    AUTHOR = {Davis, Burgess and McDonald, David},
     TITLE = {An elementary proof of the local central limit theorem},
   JOURNAL = {J. Theoret. Probab.},
  FJOURNAL = {Journal of Theoretical Probability},
    VOLUME = {8},
      YEAR = {1995},
    NUMBER = {3},
     PAGES = {693--701},
      ISSN = {0894-9840},
     CODEN = {JTPREO},
   MRCLASS = {60F05},
  MRNUMBER = {1340834 (96j:60037)},
MRREVIEWER = {Erich Haeusler},
       DOI = {10.1007/BF02218051},
       URL = {http://dx.doi.org/10.1007/BF02218051},
}
@article {MR2081491,
    AUTHOR = {Hryniv, O. and Ioffe, D.},
     TITLE = {Self-avoiding polygons: sharp asymptotics of canonical
              partition functions under the fixed area constraint},
   JOURNAL = {Markov Process. Related Fields},
  FJOURNAL = {Markov Processes and Related Fields},
    VOLUME = {10},
      YEAR = {2004},
    NUMBER = {1},
     PAGES = {1--64},
      ISSN = {1024-2953},
   MRCLASS = {60K35 (60F15 82B20 82B41)},
  MRNUMBER = {2081491 (2006b:60220)},
MRREVIEWER = {Paolo Dai Pra},
}


@article {Vy10,
    AUTHOR = {Vysotsky, Vladislav},
     TITLE = {On the probability that integrated random walks stay positive},
   JOURNAL = {Stochastic Process. Appl.},
  FJOURNAL = {Stochastic Processes and their Applications},
    VOLUME = {120},
      YEAR = {2010},
    NUMBER = {7},
     PAGES = {1178--1193},
      ISSN = {0304-4149},
     CODEN = {STOPB7},
   MRCLASS = {60G50 (60F99)},
  MRNUMBER = {2639743},
MRREVIEWER = {M. Cs{\"o}rg{\H{o}}},
       DOI = {10.1016/j.spa.2010.03.005},
       URL = {http://dx.doi.org/10.1016/j.spa.2010.03.005},
}



@article {LeGall2010,
    AUTHOR = {Le Gall, Jean-Fran{\c{c}}ois},
     TITLE = {It\^o's excursion theory and random trees},
   JOURNAL = {Stochastic Process. Appl.},
  FJOURNAL = {Stochastic Processes and their Applications},
    VOLUME = {120},
      YEAR = {2010},
    NUMBER = {5},
     PAGES = {721--749},
      ISSN = {0304-4149},
     CODEN = {STOPB7},
   MRCLASS = {60J65 (60C05 60J80)},
  MRNUMBER = {2603061},
MRREVIEWER = {Romain Abraham},
       DOI = {10.1016/j.spa.2010.01.015},
       URL = {http://dx.doi.org/10.1016/j.spa.2010.01.015},
}
		

@article {CarCha13,
    AUTHOR = {Caravenna, Francesco and Chaumont, Lo{\"{\i}}c},
     TITLE = {An invariance principle for random walk bridges conditioned to
              stay positive},
   JOURNAL = {Electron. J. Probab.},
  FJOURNAL = {Electronic Journal of Probability},
    VOLUME = {18},
      YEAR = {2013},
     PAGES = {no. 60, 32},
      ISSN = {1083-6489},
   MRCLASS = {60G50 (60F17 60G51)},
  MRNUMBER = {3068391},
MRREVIEWER = {Allan Gut},
}

@article{CP15,
author = "Carmona, Philippe and Pétrélis, Nicolas",
doi = "10.1214/16-EJP4618",
fjournal = "Electronic Journal of Probability",
journal = "Electron. J. Probab.",
pages = "52 pp.",
pno = "49",
publisher = "The Institute of Mathematical Statistics and the Bernoulli Society",
title = "Interacting partially directed self avoiding walk: scaling limits",
url = "https://doi.org/10.1214/16-EJP4618",
volume = "21",
year = "2016"
}

%@article{CP15,
%  author = 	 {Carmona, Philippe and {Pétrélis}, Nicolas},
%  title = 	 {Interacting partially directed self avoiding walk : scaling limits},
%  note = 	 {Electronic Journal of Probability},
%   VOLUME = {21},
%      YEAR = {2016},
%     PAGES = {no. 49, 1--52 (electronic)},
%      ISSN = {1083-6489},
%      DOI = {10.1214/16-EJP4618},
% }

@unpublished{CarPet17b,
  author = 	 {Carmona, Philippe and {Pétrélis}, Nicolas},
  title = 	 {Limit theorems for random walk excursion conditioned to have a typical area},
      YEAR = {2017},
 }
@unpublished{CarPet17a,
  author = 	 {Carmona, Philippe and {Pétrélis}, Nicolas},
  title = 	 {A shape theorem for the scaling limit of the IPDSAW at
criticality},
      YEAR = {2017},
 }



@article {Lachal91,
    AUTHOR = {Lachal, A.},
     TITLE = {Sur le premier instant de passage de l'int\'egrale du
              mouvement brownien},
   JOURNAL = {Ann. Inst. H. Poincar\'e Probab. Statist.},
  FJOURNAL = {Annales de l'Institut Henri Poincar\'e. Probabilit\'es et
              Statistiques},
    VOLUME = {27},
      YEAR = {1991},
    NUMBER = {3},
     PAGES = {385--405},
      ISSN = {0246-0203},
     CODEN = {AHPBAR},
   MRCLASS = {60J65 (60G15)},
  MRNUMBER = {1131839},
MRREVIEWER = {Paul McGill},
       URL = {http://www.numdam.org/item?id=AIHPB_1991__27_3_385_0},
}
	
@article {Goldman71,
    AUTHOR = {Goldman, Malcolm},
     TITLE = {On the first passage of the integrated {W}iener process},
   JOURNAL = {Ann. Mat. Statist.},
    VOLUME = {42},
      YEAR = {1971},
     PAGES = {2150--2155},
   MRCLASS = {60J60},
  MRNUMBER = {0297017},
}

@article {Kurtz91,
    AUTHOR = {Kurtz, Thomas G.},
     TITLE = {Random time changes and convergence in distribution under the
              {M}eyer-{Z}heng conditions},
   JOURNAL = {Ann. Probab.},
  FJOURNAL = {The Annals of Probability},
    VOLUME = {19},
      YEAR = {1991},
    NUMBER = {3},
     PAGES = {1010--1034},
      ISSN = {0091-1798},
     CODEN = {APBYAE},
   MRCLASS = {60F17 (60G99)},
  MRNUMBER = {1112405},
MRREVIEWER = {Adam Jakubowski},
       URL ={http://links.jstor.org/sici?sici=0091-1798(199107)19:3<1010:RTCACI>2.0.CO;2-2&origin=MSN},
}
@incollection {PitYor96,
    AUTHOR = {Pitman, Jim and Yor, Marc},
     TITLE = {Decomposition at the maximum for excursions and bridges of
              one-dimensional diffusions},
 BOOKTITLE = {It\^o's stochastic calculus and probability theory},
     PAGES = {293--310},
 PUBLISHER = {Springer, Tokyo},
      YEAR = {1996},
   MRCLASS = {60J60 (60J65)},
  MRNUMBER = {1439532},
MRREVIEWER = {F. B. Knight},
}
@incollection {MR1439532,
    AUTHOR = {Pitman, Jim and Yor, Marc},
     TITLE = {Decomposition at the maximum for excursions and bridges of
              one-dimensional diffusions},
 BOOKTITLE = {It\^o's stochastic calculus and probability theory},
     PAGES = {293--310},
 PUBLISHER = {Springer, Tokyo},
      YEAR = {1996},
   MRCLASS = {60J60 (60J65)},
  MRNUMBER = {1439532},
MRREVIEWER = {F. B. Knight},
}
@incollection {MR1478738,
    AUTHOR = {Pitman, Jim and Yor, Marc},
     TITLE = {On the relative lengths of excursions derived from a stable
              subordinator},
 BOOKTITLE = {S\'eminaire de {P}robabilit\'es, {XXXI}},
    SERIES = {Lecture Notes in Math.},
    VOLUME = {1655},
     PAGES = {287--305},
 PUBLISHER = {Springer, Berlin},
      YEAR = {1997},
   MRCLASS = {60J55 (60E99 60G99)},
  MRNUMBER = {1478738},
MRREVIEWER = {Mamoru Kanda},
       DOI = {10.1007/BFb0119314},
       URL = {http://dx.doi.org/10.1007/BFb0119314},
}
@article {VatWac09,
    AUTHOR = {Vatutin, Vladimir A. and Wachtel, Vitali},
     TITLE = {Local probabilities for random walks conditioned to stay
              positive},
   JOURNAL = {Probab. Theory Related Fields},
  FJOURNAL = {Probability Theory and Related Fields},
    VOLUME = {143},
      YEAR = {2009},
    NUMBER = {1-2},
     PAGES = {177--217},
      ISSN = {0178-8051},
   MRCLASS = {60G50 (60E07 60G52)},
  MRNUMBER = {2449127},
MRREVIEWER = {Ross S. McVinish},
       DOI = {10.1007/s00440-007-0124-8},
       URL = {http://dx.doi.org/10.1007/s00440-007-0124-8},
}
